Shisha: Online scheduling of CNN pipelines on heterogeneous architectures

Chiplets have become a common methodology in modern chip design. Chiplets improve yield and enable heterogeneity at the level of cores, memory subsystem and the interconnect. Convolutional Neural Networks (CNNs) have high computational, bandwidth and memory capacity requirements owing to the increasingly large amount of weights. Thus to exploit chiplet-based architectures, CNNs must be optimized in terms of scheduling and workload distribution among computing resources. We propose Shisha, an online approach to generate and schedule parallel CNN pipelines on chiplet architectures. Shisha targets heterogeneity in compute performance and memory bandwidth and tunes the pipeline schedule through a fast online exploration technique. We compare Shisha with Simulated Annealing, Hill Climbing and Pipe-Search. On average, the convergence time is improved by ~35x in Shisha compared to other exploration algorithms. Despite the quick exploration, Shisha's solution is often better than that of other heuristic exploration algorithms.

==> CP38_extended_references.tex <==
@inproceedings{blythe2021xehpc,
  title={XeHPC Ponte Vecchio},
  author={Blythe, David},
  booktitle={2021 IEEE HCS},
  pages={1--34},
  year={2021},
  organization={IEEE Computer Society}
}
@article{suggs2020amd,
  title={The AMD “Zen 2” Processor},
  author={Suggs, David and Subramony, Mahesh and Bouvier, Dan},
  journal={IEEE Micro},
  volume={40},
  number={2},
  pages={45--52},
  year={2020},
  publisher={IEEE}
}
@inproceedings{schone2021energy,
  title={Energy Efficiency Aspects of the AMD Zen 2 Architecture},
  author={Sch{\"o}ne, Robert and Ilsche, Thomas and Bielert, Mario and Velten, Markus and Schmidl, Markus and Hackenberg, Daniel},
  booktitle={2021 IEEE International Conference on Cluster Computing (CLUSTER)},
  pages={562--571},
  year={2021},
  organization={IEEE}
}
@article{mccalpin1995memory,
  title={Memory bandwidth and machine balance in current high performance computers},
  author={McCalpin, John D and others},
  journal={IEEE computer society technical committee on computer architecture (TCCA) newsletter},
  volume={2},
  number={19-25},
  year={1995}
}
@inproceedings{shao2019simba,
  title={Simba: Scaling deep-learning inference with multi-chip-module-based architecture},
  author={Shao, Yakun Sophia and Clemons, Jason and Venkatesan, Rangharajan and Zimmer, Brian and Fojtik, Matthew and Jiang, Nan and Keller, Ben and Klinefelter, Alicia and Pinckney, Nathaniel and Raina, Priyanka and others},
  booktitle={Proceedings of the 52nd Annual IEEE/ACM International Symposium on Microarchitecture},
  pages={14--27},
  year={2019}
}
@article{adams2019learning,
  title={Learning to optimize halide with tree search and random programs},
  author={Adams, Andrew and Ma, Karima and Anderson, Luke and Baghdadi, Riyadh and Li, Tzu-Mao and Gharbi, Micha{\"e}l and Steiner, Benoit and Johnson, Steven and Fatahalian, Kayvon and Durand, Fr{\'e}do and others},
  journal={ACM Transactions on Graphics (TOG)},
  volume={38},
  number={4},
  pages={1--12},
  year={2019},
  publisher={ACM New York, NY, USA}
}
@article{ragan2013halide,
  title={Halide: a language and compiler for optimizing parallelism, locality, and recomputation in image processing pipelines},
  author={Ragan-Kelley, Jonathan and Barnes, Connelly and Adams, Andrew and Paris, Sylvain and Durand, Fr{\'e}do and Amarasinghe, Saman},
  journal={Acm Sigplan Notices},
  volume={48},
  number={6},
  pages={519--530},
  year={2013},
  publisher={ACM New York, NY, USA}
}
@inproceedings{yang2020interstellar,
  title={Interstellar: Using halide's scheduling language to analyze dnn accelerators},
  author={Yang, Xuan and Gao, Mingyu and Liu, Qiaoyi and Setter, Jeff and Pu, Jing and Nayak, Ankita and Bell, Steven and Cao, Kaidi and Ha, Heonjae and Raina, Priyanka and others},
  booktitle={Proceedings of the Twenty-Fifth International Conference on Architectural Support for Programming Languages and Operating Systems},
  pages={369--383},
  year={2020}
}
@article{qararyah2021computational,
  title={A computational-graph partitioning method for training memory-constrained DNNs},
  author={Qararyah, Fareed and Wahib, Mohamed and Dikbay{\i}r, Do{\u{g}}a and Belviranli, Mehmet Esat and Unat, Didem},
  journal={Parallel Computing},
  volume={104},
  pages={102792},
  year={2021},
  publisher={Elsevier}
}
@inproceedings{wu2020pipeline,
  title={A Pipeline-Based Scheduler for Optimizing Latency of Convolution Neural Network Inference over Heterogeneous Multicore Systems},
  author={Wu, Hsin-I and Guo, Da-Yi and Chin, Hsu-Hsun and Tsay, Ren-Song},
  booktitle={2020 2nd IEEE International Conference on Artificial Intelligence Circuits and Systems (AICAS)},
  pages={46--49},
  year={2020},
  organization={IEEE}
}

@article{mccalpin1995stream,
  title={Stream benchmark},
  author={McCalpin, John D},
  journal={Link: www. cs. virginia. edu/stream/ref. html\# what},
  volume={22},
  pages={7},
  year={1995}
}
@inproceedings{zheng2020ansor,
  title={Ansor: Generating high-performance tensor programs for deep learning},
  author={Zheng, Lianmin and Jia, Chengfan and Sun, Minmin and Wu, Zhao and Yu, Cody Hao and Haj-Ali, Ameer and Wang, Yida and Yang, Jun and Zhuo, Danyang and Sen, Koushik and others},
  booktitle={14th $\{$USENIX$\}$ Symposium on Operating Systems Design and Implementation ($\{$OSDI$\}$ 20)},
  pages={863--879},
  year={2020}
}
@inproceedings{li2021chimera,
  title={Chimera: efficiently training large-scale neural networks with bidirectional pipelines},
  author={Li, Shigang and Hoefler, Torsten},
  booktitle={Proceedings of the International Conference for High Performance Computing, Networking, Storage and Analysis},
  pages={1--14},
  year={2021}
}
@article{ahn2020chameleon,
  title={Chameleon: Adaptive code optimization for expedited deep neural network compilation},
  author={Ahn, Byung Hoon and Pilligundla, Prannoy and Yazdanbakhsh, Amir and Esmaeilzadeh, Hadi},
  journal={arXiv preprint arXiv:2001.08743},
  year={2020}
}
@article{fedus2021switch,
  title={Switch transformers: Scaling to trillion parameter models with simple and efficient sparsity},
  author={Fedus, William and Zoph, Barret and Shazeer, Noam},
  journal={arXiv preprint arXiv:2101.03961},
  year={2021}
}
@inproceedings{li2021chimera,
  title={Chimera: efficiently training large-scale neural networks with bidirectional pipelines},
  author={Li, Shigang and Hoefler, Torsten},
  booktitle={Proceedings of the International Conference for High Performance Computing, Networking, Storage and Analysis},
  pages={1--14},
  year={2021}
}
@inproceedings{sodani2015knights,
  title={Knights landing (knl): 2nd generation intel{\textregistered} xeon phi processor},
  author={Sodani, Avinash},
  booktitle={2015 IEEE Hot Chips 27 Symposium (HCS)},
  pages={1--24},
  year={2015},
  organization={IEEE}
}
@inproceedings{AUGUR,
  title={Modeling the resource requirements of convolutional neural networks on mobile devices},
  author={Lu, Zongqing and Rallapalli, Swati and Chan, Kevin and La Porta, Thomas},
  booktitle={Proceedings of the 25th ACM international conference on Multimedia},
  pages={1663--1671},
  year={2017}
}
@article{pipeit,
  title={High-throughput cnn inference on embedded arm big. little multi-core processors},
  author={Wang, Siqi and Ananthanarayanan, Gayathri and Zeng, Yifan and Goel, Neeraj and Pathania, Anuj and Mitra, Tulika},
  journal={IEEE Transactions on Computer-Aided Design of Integrated Circuits and Systems},
  year={2019},
  publisher={IEEE}
}
@article{graphi,
  title={Scheduling computation graphs of deep learning models on manycore CPUs},
  author={Tang, Linpeng and Wang, Yida and Willke, Theodore L and Li, Kai},
  journal={arXiv preprint arXiv:1807.09667},
  year={2018}
}
@inproceedings{CSDF,
  title={Combining Task-and Data-Level Parallelism for High-Throughput CNN Inference on Embedded CPUs-GPUs MPSoCs},
  author={Minakova, Svetlana and Tang, Erqian and Stefanov, Todor},
  booktitle={International Conference on Embedded Computer Systems},
  pages={18--35},
  year={2020},
  organization={Springer}
}
@article{binkert2011gem5,
  title={The gem5 simulator},
  author={Binkert, Nathan and Beckmann, Bradford and Black, Gabriel and Reinhardt, Steven K and Saidi, Ali and Basu, Arkaprava and Hestness, Joel and Hower, Derek R and Krishna, Tushar and Sardashti, Somayeh and others},
  journal={ACM SIGARCH computer architecture news},
  volume={39},
  number={2},
  pages={1--7},
  year={2011},
  publisher={ACM New York, NY, USA}
}
@article{anderson2021efficient,
  title={Efficient automatic scheduling of imaging and vision pipelines for the GPU},
  author={Anderson, Luke and Adams, Andrew and Ma, Karima and Li, Tzu-Mao and Jin, Tian and Ragan-Kelley, Jonathan},
  journal={Proceedings of the ACM on Programming Languages},
  volume={5},
  number={OOPSLA},
  pages={1--28},
  year={2021},
  publisher={ACM New York, NY, USA}
}
@article{mullapudi2016automatically,
  title={Automatically scheduling halide image processing pipelines},
  author={Mullapudi, Ravi Teja and Adams, Andrew and Sharlet, Dillon and Ragan-Kelley, Jonathan and Fatahalian, Kayvon},
  journal={ACM Transactions on Graphics (TOG)},
  volume={35},
  number={4},
  pages={1--11},
  year={2016},
  publisher={ACM New York, NY, USA}
}
@inproceedings{soomro2021online,
  title={An online guided tuning approach to run CNN pipelines on edge devices},
  author={Soomro, Pirah Noor and Abduljabbar, Mustafa and Castrillon, Jeronimo and Peric{\`a}s, Miquel},
  booktitle={Proceedings of the 18th ACM International Conference on Computing Frontiers},
  pages={45--53},
  year={2021}
}
 @misc{ipu, title={IPU processors}, url={https://www.graphcore.ai/products/ipu}, journal={IPU Processors}, author={Ltd, Graphcore}} 
@inproceedings{fan2021dapple,
  title={DAPPLE: A pipelined data parallel approach for training large models},
  author={Fan, Shiqing and Rong, Yi and Meng, Chen and Cao, Zongyan and Wang, Siyu and Zheng, Zhen and Wu, Chuan and Long, Guoping and Yang, Jun and Xia, Lixue and others},
  booktitle={Proceedings of the 26th ACM SIGPLAN Symposium on Principles and Practice of Parallel Programming},
  pages={431--445},
  year={2021}
}
@inproceedings{narayanan2019pipedream,
  title={PipeDream: generalized pipeline parallelism for DNN training},
  author={Narayanan, Deepak and Harlap, Aaron and Phanishayee, Amar and Seshadri, Vivek and Devanur, Nikhil R and Ganger, Gregory R and Gibbons, Phillip B and Zaharia, Matei},
  booktitle={Proceedings of the 27th ACM Symposium on Operating Systems Principles},
  pages={1--15},
  year={2019}
}
@inproceedings{narayanan2021memory,
  title={Memory-efficient pipeline-parallel dnn training},
  author={Narayanan, Deepak and Phanishayee, Amar and Shi, Kaiyu and Chen, Xie and Zaharia, Matei},
  booktitle={International Conference on Machine Learning},
  pages={7937--7947},
  year={2021},
  organization={PMLR}
}
@article{huang2019gpipe,
  title={Gpipe: Efficient training of giant neural networks using pipeline parallelism},
  author={Huang, Yanping and Cheng, Youlong and Bapna, Ankur and Firat, Orhan and Chen, Dehao and Chen, Mia and Lee, HyoukJoong and Ngiam, Jiquan and Le, Quoc V and Wu, Yonghui and others},
  journal={Advances in neural information processing systems},
  volume={32},
  pages={103--112},
  year={2019}
}
@article{ben2019demystifying,
  title={Demystifying parallel and distributed deep learning: An in-depth concurrency analysis},
  author={Ben-Nun, Tal and Hoefler, Torsten},
  journal={ACM Computing Surveys (CSUR)},
  volume={52},
  number={4},
  pages={1--43},
  year={2019},
  publisher={ACM New York, NY, USA}
}
@incollection{van1987simulated,
  title={Simulated annealing},
  author={Van Laarhoven, Peter JM and Aarts, Emile HL},
  booktitle={Simulated annealing: Theory and applications},
  pages={7--15},
  year={1987},
  publisher={Springer}
}
@inproceedings{oren2021solo,
  title={SOLO: Search Online, Learn Offline for Combinatorial Optimization Problems},
  author={Oren, Joel and Ross, Chana and Lefarov, Maksym and Richter, Felix and Taitler, Ayal and Feldman, Zohar and Di Castro, Dotan and Daniel, Christian},
  booktitle={Proceedings of the International Symposium on Combinatorial Search},
  volume={12},
  number={1},
  pages={97--105},
  year={2021}
}
@INPROCEEDINGS{7383697,  author={Cho, Kyungjun and Lee, Hyunsuk and Kim, Heegon and Choi, Sumin and Kim, Youngwoo and Lim, Jaemin and Kim, Joungho and Kim, Hyungsoo and Kim, Yongju and Kim, Yunsaing},  booktitle={2015 IEEE Electrical Design of Advanced Packaging and Systems Symposium (EDAPS)},   title={Design optimization of high bandwidth memory (HBM) interposer considering signal integrity},   year={2015},  volume={},  number={},  pages={15-18},  doi={10.1109/EDAPS.2015.7383697}}
@INPROCEEDINGS{7500830,  author={Mounce, Gabriel and Lyke, Jim and Horan, Stephen and Powell, Wes and Doyle, Rich and Some, Rafi},  booktitle={2016 IEEE Aerospace Conference},   title={Chiplet based approach for heterogeneous processing and packaging architectures},   year={2016},  volume={},  number={},  pages={1-12},  doi={10.1109/AERO.2016.7500830}}

@article{10.1145/3484505,
author = {Fu, Yaosheng and Bolotin, Evgeny and Chatterjee, Niladrish and Nellans, David and Keckler, Stephen W.},
title = {GPU Domain Specialization via Composable On-Package Architecture},
year = {2021},
issue_date = {March 2022},
publisher = {Association for Computing Machinery},
address = {New York, NY, USA},
volume = {19},
number = {1},
issn = {1544-3566},
url = {https://doi.org/10.1145/3484505},
doi = {10.1145/3484505},
journal = {ACM Trans. Archit. Code Optim.},
month = {dec},
articleno = {4},
numpages = {23},
keywords = {multi-chip module, GPU computing}
}
@inproceedings{alappat2020performance,
  title={Performance Modeling of Streaming Kernels and Sparse Matrix-Vector Multiplication on A64FX},
  author={Alappat, Christie and Laukemann, Jan and Gruber, Thomas and Hager, Georg and Wellein, Gerhard and Meyer, Nils and Wettig, Tilo},
  booktitle={2020 IEEE/ACM Performance Modeling, Benchmarking and Simulation of High Performance Computer Systems (PMBS)},
  pages={1--7},
  year={2020},
  organization={IEEE}
}
@article{redmon2018yolov3,
  title={Yolov3: An incremental improvement},
  author={Redmon, Joseph and Farhadi, Ali},
  journal={arXiv preprint arXiv:1804.02767},
  year={2018}
}
@inproceedings{he2016deep,
  title={Deep residual learning for image recognition},
  author={He, Kaiming and Zhang, Xiangyu and Ren, Shaoqing and Sun, Jian},
  booktitle={Proceedings of the IEEE conference on computer vision and pattern recognition},
  pages={770--778},
  year={2016}
}
@article{li2020chiplet,
  title={Chiplet heterogeneous integration technology—Status and challenges},
  author={Li, Tao and Hou, Jie and Yan, Jinli and Liu, Rulin and Yang, Hui and Sun, Zhigang},
  journal={Electronics},
  volume={9},
  number={4},
  pages={670},
  year={2020},
  publisher={Multidisciplinary Digital Publishing Institute}
}
@ARTICLE{759349,  author={Wong, C.P. and Wong, M.M.},  journal={IEEE Transactions on Components and Packaging Technologies},   title={Recent advances in plastic packaging of flip-chip and multichip modules (MCM) of microelectronics},   year={1999},  volume={22},  number={1},  pages={21-25},  doi={10.1109/6144.759349}}
@inproceedings{kannan2015enabling,
  title={Enabling interposer-based disintegration of multi-core processors},
  author={Kannan, Ajaykumar and Jerger, Natalie Enright and Loh, Gabriel H},
  booktitle={2015 48th Annual IEEE/ACM International Symposium on Microarchitecture (MICRO)},
  pages={546--558},
  year={2015},
  organization={IEEE}
}
@inbook{10.1145/3453688.3461499,
author = {Jiao, Bo and Zhu, Haozhe and Zhang, Jinshan and Wang, Shunli and Kang, Xiaoyang and Zhang, Lihua and Wang, Mingyu and Chen, Chixiao},
title = {Computing Utilization Enhancement for Chiplet-Based Homogeneous Processing-in-Memory Deep Learning Processors},
year = {2021},
isbn = {9781450383936},
publisher = {Association for Computing Machinery},
address = {New York, NY, USA},
url = {https://doi.org/10.1145/3453688.3461499},
abstract = {This paper presents a design strategy of chiplet-based processing-in-memory systems for deep neural network applications. Monolithic silicon chips are area and power limited, failing to catch the recent rapid growth of deep learning algorithms. The paper first demonstrates a straightforward layer-wise method that partitions the workload of a monolithic accelerator to a multi-chiplet pipeline. A quantitative analysis shows that the straightforward separation degrades the overall utilization of computing resources due to the reduced on-chiplet memory size, thus introducing a higher memory wall. A tile interleaving strategy is proposed to overcome such degradation. This strategy can segment one layer to different chiplets which maximizes the computing utilization. To facilitate the strategy, the modification of the chiplet system hardware is also discussed. To validate the proposed strategy, a nine-chiplet processing-in-memory system is evaluated with a custom-designed object detection network. Each chiplet can achieve a peak performance of 204.8GOPS at a 100-MHz rate. The peak performance of the overall system is 1.711TOPS, where no off-chip memory access is needed. By the tile interleaving strategy, the utilization is improved from 53.9 to 92.8},
booktitle = {Proceedings of the 2021 on Great Lakes Symposium on VLSI},
pages = {241–246},
numpages = {6}
}

@inproceedings{zhang-hpdc14-toppim,
author = {Zhang, Dongping and Jayasena, Nuwan and Lyashevsky, Alexander and Greathouse, Joseph L. and Xu, Lifan and Ignatowski, Michael},
title = {TOP-PIM: Throughput-Oriented Programmable Processing in Memory},
year = {2014},
isbn = {9781450327497},
publisher = {Association for Computing Machinery},
address = {New York, NY, USA},
url = {https://doi.org/10.1145/2600212.2600213},
doi = {10.1145/2600212.2600213},
abstract = {As computation becomes increasingly limited by data movement and energy consumption, exploiting locality throughout the memory hierarchy becomes critical to continued performance scaling. Moving computation closer to memory presents an opportunity to reduce both energy and data movement overheads. We explore the use of 3D die stacking to move memory-intensive computations closer to memory. This approach to processing in memory addresses some drawbacks of prior research on in-memory computing and is commercially viable in the foreseeable future.Because 3D stacking provides increased bandwidth, we study throughput-oriented computing using programmable GPU compute units across a broad range of benchmarks, including graph and HPC applications. We also introduce a methodology for rapid design space exploration by analytically predicting performance and energy of in-memory processors based on metrics obtained from execution on today's GPU hardware. Our results show that, on average, viable PIM configurations show moderate performance losses (27%) in return for significant energy efficiency improvements (76% reduction in EDP) relative to a representative mainstream GPU at 22nm technology. At 16nm technology, on average, viable PIM configurations are performance competitive with a representative mainstream GPU (7% speedup) and provide even greater energy efficiency improvements (85% reduction in EDP).},
booktitle = {Proceedings of the 23rd International Symposium on High-Performance Parallel and Distributed Computing},
pages = {85–98},
numpages = {14},
keywords = {performance modeling and analysis, energy efficiency, processing in memory, gpgpu},
location = {Vancouver, BC, Canada},
series = {HPDC '14}
}
